Interference Power Bound Analysis of a Network of Wireless Robots

We consider a fundamental problem concerning the deployment of a wireless robotic network: to fulfill various end-to-end performance requirements, a "sufficient" number of robotic relays must be deployed to ensure that links are of acceptable quality. Prior work has not addressed how to find this number. We use the properties of Carrier Sense Multiple Access (CSMA) based wireless communication to derive an upper bound on the spacing between any transmitter-receiver pair, which directly translates to a lower bound on the number of robots to deploy. We focus on SINR-based performance requirements due to their wide applicability. Next, we show that the bound can be improved by exploiting the geometrical structure of a network, such as linearity in the case of flow-based robotic router networks. Furthermore, we also use the bound on robot count to formulate a lower bound on the number of orthogonal codes required for a high probability of interference free communication. We demonstrate and validate our proposed bounds through simulations.

==> figures/fig1 <==
\resizebox {\columnwidth} {!}{ 
\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
]
\node[squarednode]      (source1)    at  (-5,0)  {$Src_k$};
\node[squarednode]      (sink)   at  (5,0) {$Sink_k$};
\node[roundnode]      (r2)  at  (1,-1) {$r_3$};
\node[roundnode]      (r4)  at  (4,1) {$r_5$};
\node[roundnode]      (r3)  at  (2,-3) {$r_4$};
\node[roundnode]      (r1)  at  (-3.5,-3) {$r_1$};
\node[roundnode]      (r5)  at  (-1,2) {$r_2$};
\draw[dashed] (source1.east) -- (sink.west);
\draw[dashed] (r1.north) -- (-3.5,0);
\draw[dashed] (r2.north) -- (1,0);
\draw[dashed] (r3.north) -- (2,0);
\draw[dashed] (r4.south) -- (4,0);
\draw[dashed] (r5.south) -- (-1,0);
\node at (r1.south) [below] {$RCV(r_1)=r_2$, $SRM(r_1)=Src_k$};
\node at (r2.south) [below] {$RCV(r_3)=r_4$, $SRM(r_3)=r_2$};
\node at (r3.south) [below] {$RCV(r_4)=r_5$, $SRM(r_4)=r_3$};
\node at (r4.north) [above] {$RCV(r_5)=Sink_k$, $SRM(r_5)=r_4$};
\node at (r5.south) [below] {$RCV(r_2)=r_3$, $SRM(r_2)=r_1$};

\end{tikzpicture}
}

==> figures/lemma2 <==
\resizebox {\columnwidth} {!}{ 
\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=3cm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5cm},
]

\node[roundnode] (r1)  at  (0,0) {$r_2$};
\draw[thick] (1.5,-3) -- (1.5,3);
\draw[thick] (1.5,-3) -- (1.5,3);
\end{tikzpicture}
}

==> figures/path_illus <==
\resizebox {\columnwidth} {!}{ 
\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
]
\node[squarednode]      (src)  at  (-5,0) {$Src$};
\node[roundnode]      (r1)  at  (-3,0) {$r_1$};
\node[roundnode]      (r2)  at  (-1,0) {$r_2$};
\node[roundnode]      (r3)  at  (1,0) {$r_3$};
\node[roundnode]      (r4)  at  (3,0) {$r_4$};
\node[squarednode]      (sink)  at  (5,0) {$Sink$};

\draw (src.east) -- (r1.west);
\draw (r1.east) -- (r2.west);
\draw (r2.east) -- (r3.west);
\draw (r3.east) -- (r4.west);
\draw (r4.east) -- (sink.west);
\draw[dashed] (src.south) .. controls (-5,-1) and (-1,-1) ..  (r2.south);
\draw[dashed] (r1.north) .. controls (-3,1) and (1,1) ..  (r3.north);
\draw[dashed] (r2.south) .. controls (-1,-1) and (3,-1) ..  (r4.south);
\draw[dashed] (r3.north) .. controls (1,1) and (5,1) ..  (sink.north);

\end{tikzpicture}
}

==> figures/reallocation1 <==
\resizebox {0.8\columnwidth} {!}{ 
\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
]
\node[squarednode]      (src)  at  (-5,0) {$Src$};
\node[roundnode]      (r1)  at  (-3,0) {$r_1$};
\node[roundnode]      (r2)  at  (-1,0) {$r_2$};
\node[roundnode]      (r3)  at  (1,0) {$r_3$};
\node[roundnode]      (r4)  at  (3,0) {$r_4$};
\node[squarednode]      (sink)  at  (5,0) {$Sink$};

\draw (src.east) -- (r1.west);
\draw (r1.east) -- (r2.west);
\draw (r2.east) -- (r3.west);
\draw (r3.east) -- (r4.west);
\draw (r4.east) -- (sink.west);
\draw[->] (r2.north) -- (-1,1);
\end{tikzpicture}
}

==> figures/reallocation2 <==
\resizebox {0.8\columnwidth} {!}{ 
\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
]
\node[squarednode]      (src)  at  (-5,0) {$Src$};
\node[roundnode]      (r1)  at  (-2.5,0) {$r_1$};
\node[roundnode]      (r2)  at  (-1,1) {$r_2$};
\node[roundnode]      (r3)  at  (0.5,0) {$r_3$};
\node[roundnode]      (r4)  at  (3,0) {$r_4$};
\node[squarednode]      (sink)  at  (5,0) {$Sink$};

\draw (src.east) -- (r1.west);
\draw (r1.north) -- (r2.west);
\draw (r2.east) -- (r3.north);
\draw (r3.east) -- (r4.west);
\draw (r4.east) -- (sink.west);
\draw (r1.east) -- (r3.west);
\draw[->] (r2.north) -- (-1,2);

\end{tikzpicture}
}

==> figures/reallocation3 <==
\resizebox {0.8\columnwidth} {!}{ 
\begin{tikzpicture}[
roundnode/.style={circle, draw=green!60, fill=green!5, very thick, minimum size=7mm},
squarednode/.style={rectangle, draw=red!60, fill=red!5, very thick, minimum size=5mm},
]
\node[squarednode]      (src)  at  (-5,0) {$Src$};
\node[roundnode]      (r1)  at  (-2.5,0) {$r_1$};
\node[roundnode]      (r2)  at  (-1,2) {$r_2$};
\node[roundnode]      (r3)  at  (0,0) {$r_3$};
\node[roundnode]      (r4)  at  (2.5,0) {$r_4$};
\node[squarednode]      (sink)  at  (5,0) {$Sink$};

\draw (src.east) -- (r1.west);
\draw (r3.east) -- (r4.west);
\draw (r4.east) -- (sink.west);
\draw (r1.east) -- (r3.west);
\draw[->] (r2.north) -- (-1,3);

\end{tikzpicture}
}
